On the Use of Static Analysis to Engage Students with Software Quality Improvement: An Experience with PMD

Static analysis tools are frequently used to scan the source code and detect deviations from the project coding guidelines. Given their importance, linters are often introduced to classrooms to educate students on how to detect and potentially avoid these code anti-patterns. However, little is known about their effectiveness in raising students awareness, given that these linters tend to generate a large number of false positives. To increase the awareness of potential coding issues that violate coding standards, in this paper, we aim to reflect on our experience with teaching the use of static analysis for the purpose of evaluating its effectiveness in helping students with respect to improving software quality. This paper discusses the results of an experiment in the classroom over a period of 3 academic semesters, involving 65 submissions that carried out code review activity of 690 rules using PMD. The results of the quantitative and qualitative analysis shows that the presence of a set of PMD quality issues influence the acceptance or rejection of the issues, design, and best practices-related categories that take a longer time to be resolved, and students acknowledge the potential of using static analysis tools during code review. Through this experiment, code review can turn into a vital part of the educational computing plan. We envision our findings enabling educators to support students with code review strategies to raise students awareness about static analysis tools and scaffolding their coding skills.

==> Sections/08_implication.tex <==
\section{\textcolor{blue}{Implications}}
\label{Section:Implication}
\subsection{\textcolor{blue}{Implications for Educators}}
\begin{itemize}
    \item \textcolor{blue}{\textbf{Active learning}. It refers to the instructional method that engages students in
    the learning process. From a pedagogical perspective, code review is considered an active learning technique in SE education as it is a team activity and requires technical knowledge during the code review and analysis \cite{hilburn2011read,chong2021assessing}. Our first and third research question show how students are being challenged in comprehending code and fixing the issues. To cope with this challenge and develop students' critical and analytical skills, educators can consider performing the following activities: (1) advocate to follow agile practice (Test-driven development (TDD) approach) to reproduce ASAT issues, (2) teach best practices for quality improvement, using metrics, and performing refactorings, (3) provide students with complementary tools for issues detection and correction, (4) teach to providing constructive criticism to others during code review, and (5) guide to providing instructions of how to construct useful descriptive comments.}
      \item \textcolor{blue}{\textbf{Cooperative learning.} It refers to the teaching methods in which students work in small groups to
assist one another in learning the content.  We observe from Figure \ref{fig:boxplot} that `Design' and `Best Practices' take longer to be resolved due to the fact that resolving quality issues might require effective correction measures. To facilitate the resolution time and increase students' engagement, we recommend applying the following tasks: (1) advocate for students to contribute to an open source project to fix issues as it has been shown that this helps  improving students technical skills
and self-confidence \cite{pinto2019training}, (2) experience students with coming to a consensus during code review in cases opinions differ, and (3) engage students in early computing courses in the peer code review process.}
     \item \textcolor{blue}{\textbf{Interactive learning.} It refers to the activities where students start interacting using tools and receive instant feedback. One of our main goals is to teach creativity in code review which can further enhance problem-solving abilities as well as an understanding of potential coding issues that violate coding standards. To do so, we recommend educators engage students with an interactive ASAT to provide instant feedback as part of the existing development workflow.}
    
    \item \textcolor{blue}{\textbf{Research-based learning.} It refers to the activities that connect teaching with research, which allows the inclusion of students in an investigation and execution of an experiment. Integrating research with teaching strengthens students learning outcomes as they can participate in using several ASATs, and compare, contrast and report their findings.}  
\end{itemize}

\subsection{\textcolor{blue}{Implications for Researchers \& Tool Builders}}

\subsection{\textcolor{blue}{Implications for Practitioners}}

==> Tables/Statistics.tex <==
\begin{table}
  \centering
  %\fontsize{8}{9}\selectfont
	%\tabcolsep=0.05cm
	 \caption{Dataset overview.}
	 \label{Table:Statistics}
%\begin{sideways}
%\begin{adjustbox}{width=0.48\textwidth,center}
%\begin{adjustbox}{width=\textheight,totalheight=\textwidth,keepaspectratio}
\begin{tabular}{lclllll}\hline
\toprule
\bfseries Item & \bfseries Count    \\
\midrule
No. of students &  95 \\
Completed assignments & 65 \\
No. of selected issues  &  690 \\
No. of selected distinct issues  &  155 \\
No. of true positive distinct issues & 89 \\
No. of false positive distinct issues & 9 \\
No. of true and false positive distinct issues & 57 \\
\bottomrule
\end{tabular}
%\end{adjustbox}
%\end{sideways}
\vspace{-.3cm}
\end{table}
